Inner product formula for Yoshida lifts

We prove an explicit inner product formula for vector-valued Yoshida lifts. As a consequence, we obtain the non-vanishing of Yoshida lifts.

==> Heckop.tex <==
% !TEX root = yoshidanorm.tex

\subsection{Hecke eigenvalues of the Yoshida lift}Hereafter, 
we denote by $\pi$ the automorphic representation of $D^\times_\A$ associated with $\bff$. 
If $F=\Q\times \Q$, 
the automorphic form $\bff$ is a pair $(\bff_1, \bff_2)$ of automorphic forms on $D^\times_{0,\A}$ 
associated with $\bff_i$ for $i=1,2$. 
We also define $\Pi$ to be the automorphic representation of ${\rm GSp}_4(\A)$ 
associated with $\theta(\varphi, \bff)$. 
We write the decomposition to the restricted tensor product of $\pi$ 
as $\pi=\ot^\prime_v\pi_v$. 
We use the similar notation for $\pi_1, \pi_2$ and $\Pi$. It is well known that $\theta(\test,\bff^\dag)$ is an eigenform of Hecke operators $T_1(p)$ and $T_2(p)$ at $p\ndivides N_F$. 
In this subsection, we show that $\theta(\test,\bff^\dag)$ is also an eigenform of the $U_1(p)$-operators for $p|N_F$ and compute their eigenvalues. First we call the definition of certain Hecke operators.\begin{align*}
 T_1(p) =& {\rm GSp}_4(\Z_p) {\rm diag}(p,p,1,1) {\rm GSp}_4(\Z_p), 
 \quad  T_2(p) = {\rm GSp}_4(\Z_p) {\rm diag}(p,p^2,p,1) {\rm GSp}_4(\Z_p), \\
 U_1(p) =& \Gamma_0(p) {\rm diag}(p,p,1,1) \Gamma_0(p).    
\end{align*}
For $K={\rm GSp}_4(\Z_p)$ or $\Gamma_0(p)$ and $h\in M_4(\Z_p)\cap {\rm GSp}_4(\Q_p)$, we decompose 
\begin{align*}
K h K  = \coprod_i h_i K.   
\end{align*}
Then, we define an action of 
a double coset $KhK$ on 
 a cusp form $F$ on ${\rm GSp}_4({\A})$ of level $\Gamma_0(N)$ to be  
\begin{align*}
  [KhK] (F) (g) = \sum_i F(g h_i), 
\end{align*}
where if $p\nmid N$ (resp. $p\mid N$), then $K={\rm GSp}_4(\Z_p)$ (resp. $\Gamma_0(p)$).
For $p\mid N$,  we also define the Atkin-Lehner operator $W_p$ to be  
\begin{align*}
    W_p F(g) = F(g \pMX{}{-\bfone_2}{p^{e_p}\bfone_2}{} ), 
    \quad e_p:={\rm ord}_p(N).
\end{align*}
In the rest of this subsection, we describe the action of $T_1(p), T_2(p), U_1(p)$ and $W_p$ 
on Yoshida lifts $\theta(\varphi, \bff ^\dag)$. 

Firstly, we compute the action of double cosets. 

\begin{lem}\label{heckedecomp}
We have the following decompositions:
\begin{align*}
   U_1(p) =& \coprod_{X\in {\rm Sym}_2(\Z/p\Z)} 
                     \pMX{p\bfone_2}{X}{}{\bfone_2} 
                    \Gamma_0(p).
\end{align*}
\end{lem}
\begin{proof}
The decomposition in the statement follows from a similar arguments 
given in \cite[Section 6.1]{rs07}.
\end{proof}

\begin{lem}\label{thetazero}
Let $p$ be a prime dviding $N^+$ and split in $F/{\Q}$.    
For $t\in H^0(\Q_p)$, let $\varphi^t_{p}$ be  
 the characteristic function of  $t {\rm M}_2(\Z_p)^{\oplus 2} t^{-1}$. 
Put $\varphi^t= \otimes_{v\neq p}\test_v \otimes \varphi^t_p$. 
Then,  $\theta(\varphi^t, \bff ^\dag)$ is vanishing. 
\end{lem}
\begin{proof}
We may assume that $g \in {\rm Sp}_4({\A})$. 
By the definition of theta series, we find that 
\begin{align*}
   \theta(\varphi^t, \bff ^\dag) (g)
 = & \int_{[H^0_1]}   \sum_{x \in \bfX}  
         \langle \omega(h, g)\varphi^t(x), \bff ^\dag(h)  \rangle_\cW dh  \\ 
 = & \sum_{x \in  H^0_1({\Q})\backslash\bfX} 
       \sum_{\gamma \in H^0_1({\Q})}
          \int_{[H^0_1]}    
         \langle \omega(\gamma h, g)\varphi^t(x), 
          \bff ^\dag( \gamma h)  \rangle_\cW dh  \\ 
 = & \sum_{x \in  H^0_1({\Q})\backslash\bfX} 
          \int_{H^0_1({\A})}    
         \langle \omega( h, g)\varphi^t(x), 
          \bff ^\dag(  h)  \rangle_\cW dh.
\end{align*}  
We denote $\wh{R}^\times_{\frakN^+}$ by $\cU$ 
 and  write  $\cU=\prod_v \cU_v$. 
Define $\wtd{\cU}_p = {\rm GL}_2(\Z_p) \times_{\Z^\times_p} 
                                  {\rm GL}_2(\Z_p) \subset H^0(\Q_p)$. 
We also define 
$\wtd{\cU}=\wtd{\cU}_p\times \prod_{v\neq p} \cU_v$.   
Then, for each $u \in t^{-1} \wtd{\cU} t$, we find that $\varphi^t(u^{-1} x) = \varphi^t(x)$.      
Hence, we obtain 
\begin{align*}
    &   \int_{H^0_1(\A)}    
         \langle \omega( h, g)\varphi^t(x), 
          \bff ^\dag(  h)  \rangle_\cW dh    \\ 
  =& {\rm vol}(dh, \cU \cap t^{-1} \cU t)   
        \int_{H^0_1(\A) / t^{-1 } \wtd{\cU} t }    
        \sum_{u \in t^{-1} \wtd{\cU} t / \cU \cap t^{-1} \cU t}         
         \langle \omega( h u, g)\varphi^t(x), 
          \bff ^\dag(  h u)  \rangle_\cW dh  \\   
  =& {\rm vol}(dh, \cU \cap t^{-1} \cU t)   
        \int_{H^0_1(\A) / t^{-1 } \wtd{\cU} t }          
         \langle \omega( h , g)\varphi^t(x), 
       \sum_{u \in  \wtd{\cU}  / t \cU t^{-1} \cap \cU }   
          \bff ^\dag(  h t^{-1} u t)  \rangle_\cW dh.    
\end{align*}
Define 
$\widetilde\bff ^\dag (h)
  = \sum_{u \in  \wtd{\cU}  / t \cU t^{-1} \cap \cU }   
          \bff ^\dag(  h  u t)$ for $h\in H^0(\A)$.
Then, we have 
$\widetilde\bff ^\dag(h\wtd{u}) = \wtd{\bff} ^\dag(h)$ 
for each $\wtd{\cU}$.
Since $\pi$ has no non-trivial $\wtd{\cU}$-invariant vector, 
  $\wtd{\bff} ^\dag $ have to be zero.   
This proves $\theta( \varphi^t, \bff ^\dag) =0$. 
\end{proof}


\begin{prop}\label{thetaeigen}
We denote by $\bar{\ast}$ the complex conjugate of $\ast$.
Let $c(f_i)_{p}$ be the Hecke eigenvalue of $f$ at $p$ $(i=1,2)$.
\begin{enumerate}
\item \label{thetaeigen(1)}
  For $i=1,2$, the theta series $\theta(\test, \bff ^\dag)$ is an eigen form of $T_i(p)$ 
    for $p\nmid N$.
    In particular, we have  
\begin{align*}
T_1(p) ( \theta(\test, \bff ^\dag) ) 
     =& \theta(\test, \bff ^\dag) \times 
              \begin{cases} p(\bar{ c(f_1)_p} + \bar{c(f_2)_p }),   & p: \text{split in } F/\Q, \\
                                                                       0, & p:\text{non-split in } F/\Q, \end{cases} \\ 
T_2(p) (\theta(\test, \bff ^\dag) ) 
      =& \theta(\test, \bff ^\dag) \times  
                                                    \begin{cases}  ((p^2-1)+ p\bar{ c(f_1)_p}  \bar{c(f_2)_p }), & p: \text{split in } F/\Q,  \\ 
                                                                          -(p^2+1 + p c(f)_p ), & p:\text{non-split in } F/\Q. \end{cases} 
\end{align*}
\item \label{thetaeigen(2)}
Assume that $p$ is split in $F/\Q$ and $p$ divides {\rm l.c.m.}($N_1, N_2$). 
If $p \mid N_i$ for $i=1$ or $2$, 
   we write $\pi=\sigma(\mu_i |\cdot|^\frac{1}{2}, \mu_i |\cdot|^{-\frac{1}{2}})$. 
Then, we have 
\begin{align*}
U_1(p) ( \theta(\test, \bff ^\dag) ) 
   =& \theta(\test, \bff ^\dag) \times 
          \begin{cases} p\mu_1(p) = p\mu_2(p),  & p\mid {\rm g.c.d.}(N_1, N_2), \pi_{1,p}\cong \pi_{2,p},  \\
                                  p\mu_1(p), & p\mid N_1, p\nmid N_2, \\
                                 p\mu_2(p), & p\nmid N_1, p\mid N_2.   \end{cases} 
\end{align*}
\item \label{thetaeigen(3)}
If $p$ is non-split in $F/\Q$, we have 
\begin{align*}
U_1(p) (\theta(\test, \bff ^\dag))  =& pW_p( \theta(\test, \bff ^\dag)),  
\quad  U_1(p) (W_p(\theta(\test, \bff ^\dag) ) )  = p \theta(\test, \bff ^\dag).  
\end{align*}
\end{enumerate}
\end{prop}
\begin{proof}
The first statement follows from 
   \cite[Theorem 5.1]{yo80}  (resp. \cite[Theorem 5.2, Remark 5.3]{yo80})
if $p$ is split (resp. non-split and odd) in $F/\Q_p$.
In the case that $p=2$ is non-split in $F/\Q_p$, 
the statement for $T_i(p)$ is \cite[p.543, Main Theorem]{jlr12}.

We prove the second statement. 
We suppose that $p$ divides $N$, since the other case is prove in the same way. 
Let $\eta_p=\pMX{0}{1}{-p}{0}$ and $h_0 = (\bfone_2,\eta_p^{-1}) \in H^0(\Q_p)$. 
Note that we have $\nu(h_0)=p$. 
By the definition of theta series and Lemma \ref{heckedecomp}, 
we find that 
\begin{align*}
U_1(p)\theta(\test,\bff^\dag)(g)&=\int_{[H^0_1]}\sum_{B\in {\rm S}_2(\Zp/p\Zp)}\pair{\theta(hh'h_0;g\pMX{p\bfone_2}{B}{0}{\bfone_2}\test)}{\bff^\dag(hh'h_0}_\cW\rmd h\\
&=\theta(\varphi',\rho(h_0)\bff^\dag)(g),
\end{align*}
where $\rho(h_0)\bff^\dag(h)=\bff^\dag(hh_0)$ and 
\[\varphi':=\sum_{B\in {\rm Sym}_2(\Z/p\Z)}\om_p(h_0,\pMX{p\bfone_2}{B}{0}{\bfone_2})\test.\]
where $h^\prime \in H({\A})$ such that  $\nu(h^\prime) = \nu(g)$.
If $B=\pMX{a}{b}{b}{c}\in{\rm Sym_2}(\Zp)$, then we have \begin{align}
   \omega_p(h_0, \pMX{p\bfone_2}{B}{0}{\bfone_2})
     \test_p(x)                  
 =&  p^2 \cdot \omega_{V_p} (   \pMX{p\bfone_2}{}{}{p^{-1}\bfone_2} 
                                          \pMX{\bfone_2}{p^{-1}B }{}{ \bfone_2 } )
     \test_p(h^{-1}_0 x)   \notag  \\
 =& p^{-2}\psi_p(a {\rm n}(x_1) + \rpair{x_1}{x_2} + c {\rm n}(x_2) )
      \test_p(x_1\eta_p,x_2\eta_p ).  \label{weilactp}
\end{align}
We find that
\[\varphi'(x_1,x_2)=\sum_{a,b,c}\psi_p(a{\rm n}(x_1)+b\rpair{x_1}{x_2}+c{\rm n}(x_2))\test(x_1\eta_p,x_2\eta_p).\]
Then $(x_1,x_2)\in\supp\varphi'$ if and only if $x_1,x_2\in R_0\eta_p^{-1}$, ${\rm n}(x_1)\in\Zp$, 
$\rpair{x_1}{x_2}\in\Zp$ and ${\rm n}(x_2)\in\Zp$. Recall that $\test_p$ is the characteristic function of 
$L_p:=R_0\oplus R_0$, where $R_0=\pMX{\Zp}{\Zp}{p\Zp}{\Zp}$. For $x\in {\rm M}_2(\Qp)$, $x\eta_p\in R_0$ if and only if \begin{align*}
   x \in L':=\pMX{\Z_p}{p^{-1}\Z_p}{\Z_p}{\Z_p}.  
\end{align*}
Define lattices $L_1,L_2$ by 
\[L_1=\pMX{\Z_p}{\Z_p}{\Z_p}{\Z_p};\quad  L_2=\pMX{\Z_p}{p^{-1}\Z_p}{p\Z_p}{\Z_p}.\]
Then for $(x_1,x_2)\in L'\oplus L'$, 
\begin{align*}{\rm n}(x_1),\,{\rm n}(x_2)\in\Zp\iff &x_1,x_2\in L_1\cup L_2;\\
(x_1,x_2)\in \Zp\iff& (x_1,x_2)\in L_1\oplus L_1\text{ or }L_2\oplus L_2.
\end{align*}
Therefore, we find that 
\[\varphi'(x)=\bbI_{L_1\oplus L_2}+\bbI_{L_2\oplus L_2}-\bbI_{R_0\oplus R_0}.\]

Hence, we find that 
\begin{align*}
     \sum_{ \substack{ a, b, c \\ {\rm mod} \ p } }  
        p^{-2} \psi_p(a {\rm n}(x_1) + b(x_1, x_2) + c {\rm n}(x_2) )
        \test_p( h_0x_1, h_0x_2 )
   = p({\mathbb I}_{\tilde{L}^{\oplus 2}_1}(x) + {\mathbb I}_{\tilde{L}^{\oplus 2}_2}(x) 
            - {\mathbb I}_{(\tilde{L}_1 \cap \tilde{L}_2 )^{\oplus 2}}(x)  ).  
\end{align*}
Put $\varphi^{(p)} = \otimes_{v\neq p} \test_v$. 
Then, by Lemma \ref{thetazero}, we find that, for $i=1,2$,  
\begin{align*}
  \theta(g; \varphi^{(p)} {\mathbb I}_{L^{\oplus 2}_i}, \bff ^\dag) =0. 
\end{align*} 
Since ${\mathbb I}_{(\tilde{L}_1 \cap \tilde{L}_2 )^{\oplus 2}} = \test_p$, we obtain 
\begin{align*}
  U_1(p) (\theta(g; \test, \bff ^\dag)) 
  = -p (g; \test, \bff ^\dag|_{h_0}),  
\end{align*}   
where we define $\bff ^\dag|_{h_0}(h) = \bff ^\dag(hh_0)$.   
By \cite[3.1.2 Proposition]{sc02}, we find that 
$\bff ^\dag|_{h_0} = -\mu_1(p) \bff ^\dag$.
This proves the second statement. 

We prove the third statement. 
In the similar way as above, 
we compute 
\begin{align*}
    U_1(p) ( \theta(g; \test, \bff ^\dag) ) 
 =& \sum_{ X\in S_2(\Z/p\Z)} 
      \int_{[H^0_1]} \sum_{x \in \bfX} 
      \langle \omega(hh^\prime, 
                                 g    \pMX{\bfone_2}{ X}{}{\bfone_2} 
                                         \pMX{p\bfone_2}{}{}{\bfone_2}  )  
      \test(x),
      \bff ^\dag(hh^\prime) 
      \rangle_\cW dh,
\end{align*}
where $h^\prime \in H^0({\A})$ such that  $\nu(h^\prime) = \nu(g)$.
We note the following identity:
\begin{align*}
   \pMX{\bfone_2}{ \pMX{a}{b}{b}{c} }{}{\bfone_2} 
   \pMX{p\bfone_2}{}{}{\bfone_2} 
= \pMX{}{-\bfone_2}{p\bfone_2}{} 
   \pMX{}{\bfone_2}{-\bfone_2}{} 
   \pMX{p\bfone_2}{}{}{p^{-1}\bfone_2} 
   \pMX{\bfone_2}{ p^{-1} \pMX{a}{b}{b}{c} }{}{\bfone_2}. 
\end{align*}
We compute the following action of the Weil representation:
\begin{align*}
 & \omega_{V_p}(
   \pMX{}{\bfone_2}{-\bfone_2}{} 
   \pMX{p\bfone_2}{}{}{p^{-1}\bfone_2} 
    \pMX{\bfone_2}{  p^{-1} \pMX{a}{b}{b}{c} }{}{ \bfone_2 }  ) 
    \test_p(x_1, x_2) \\
 =&p^{-4}  \omega_{V_p}( \pMX{}{\bfone_2}{-\bfone_2}{} ) 
       \psi_p( p ( a{\rm n}(x_1) + b(x_1, x_2) + c{\rm n}(x_2)  ) )
      \test_p(px_1, px_2).   
\end{align*}
By the similar argument in the proof of the second statement, 
   we find that 
\begin{align*}
  \sum_{ \substack{ a, b, c \\ {\rm mod}\ p } }  
   p^{-4} \psi_p( p ( a{\rm n}(x_1) + b(x_1, x_2) + c{\rm n}(x_2)  ) )
      \test_p(px_1, px_2)
 = p^{-1} {\mathbb I}_{\tilde{L}^{\oplus 2}}(x),  
\end{align*}   
where $\tilde{L} =\pMX{\cO_p}{p^{-1}\Z_p}{\Z_p}{\cO_p} \cap V_p$. 
It is easy to see that 
\begin{align*}
 \omega_{V_p}( \pMX{}{\bfone_2}{-\bfone_2}{} )({\mathbb I}_{\tilde{L}^{\oplus 2}})
 = p^2 \test_p.   
\end{align*}
Hence, we obtain
\begin{align*}
    U_1(p) ( \theta(g; \test, \bff ^\dag) ) 
 = p \sum_{ \substack{ a, b, c \\ {\rm mod}\ p } } 
      \int_{[H^0_1]} \sum_{x \in \bfX} 
      \langle \omega(hh^\prime, 
                                g   \pMX{}{-\bfone_2}{p\bfone_2}{}  )\test(x), 
                                \bff ^\dag(hh^\prime) \rangle_\cW dh
 = pW_p ( \theta(g; \test, \bff ^\dag) ).
\end{align*}
This proves the third statement. 
\end{proof}

\begin{rem}\label{U(p)evrem}
Let  $\Pi\cong \otimes^\prime_v \Pi_v$ 
be the cuspidal automorphic  representation of ${\rm GSp}_4({\A})$ 
attached to $\theta(\test, \newform )$. 
We compare Proposition \ref{thetaeigen} with 
some representation theoretic properties of $\Pi_p$
 which are described in \cite{rs07} and \cite{sc05}. 
We use notation of \cite[Table A.1]{rs07} and \cite[Table 1]{jlr12} 
for irreducible admissible representations of ${\rm GSp}_4(\Q_p)$.
\begin{enumerate}
\item If $p\mid N$ is split, then by \cite[Table 1]{jlr12} and \cite[Theorem A.9, Theorem A.10]{gi11}, 
         we find that $\Pi_p$ is isomorphic 
          to either (IIa), (IVc), (Va), (Vb$^\ast$),   (VIa) or (VIb). 
         By \cite[Table A. 15]{rs07} and \cite[2.6 Proposition]{ca80}, we find that          
         \begin{align*}
            \dim_{\C} \Pi^{\Gamma_0(p)}_p 
            = \begin{cases}   1, &  \text{if } \Pi_p  \text{ is type (IIa), (IVc), (VIa), (VIb)}, \\
                                        0,  &  \text{if } \Pi_p \text{ is type (Va), (Vb$^\ast$)}.   \end{cases}
         \end{align*}
         Hence, if $\Pi_p$ is either type (IIa), (IVc), (VIa) or (VIb), 
         then we can also deduce Proposition \ref{thetaeigen}(\ref{thetaeigen(2)}) by 
         \cite[(24)]{sc05}. 
         If $\Pi_p$ is either type (Va) or (Vb$^\ast$), 
         then $p\mid {\rm g.c.d}(N_1, N_2)$ and $\pi_{1,p} \not\cong \pi_{2,p}$. 
         Hence, it is necessary to consider this case in Proposition \ref{thetaeigen}(\ref{thetaeigen(2)}).
\item If $p\mid N$ is inert,  then by \cite[Table 1]{jlr12} and \cite[Theorem A.11]{gi11}, 
         we find that $\Pi_p$ is isomorphic 
          to either (IIIa) or (Va). 
         By \cite[Table A. 15]{rs07}, we find that          
         \begin{align*}
            \dim_{\C} \Pi^{\Gamma_0(p)}_p 
            = \begin{cases}   2, &  \text{if } \Pi_p  \text{ is type (IIIa)}, \\
                                        0,  &  \text{if } \Pi_p \text{ is type (Va)}.   \end{cases}
         \end{align*} 
         By \cite[(24)]{sc05}, we find that, if $\Pi_p$ is  type (IIIa), then 
         the characteristic polynomial of $U_1(p)$ is given by 
         $X^2-p^2$, where $X$ is an indeterminate. 
         This is compatible with  Proposition \ref{thetaeigen}(\ref{thetaeigen(3)}).
\end{enumerate}
\end{rem}


We compute the action of Atkin-Lehner operator $W_p$ on Yoshida lifts as follows:

\begin{prop}\label{ALTheta}
 Suppose that $p\mid N_D$ is split in $F/{\Q}$.  
We denote by $\ep(\pi_{i,p}) \in \{\pm 1\}$ the local root number of $\pi_{i,p}$ . 
Then, there exists $\varepsilon_p(\theta(\test, \bff ^\dag) ) \in \{\pm 1\}$ such that 
\begin{align*}
    W_p \theta(\test, \bff ^\dag) = \varepsilon_p(\theta(\test, \bff ^\dag)) \theta(\test, \bff ^\dag).
\end{align*}
Furthermore,the values $\varepsilon_p(\theta(\test, \bff ^\dag) )$ are given as follows
\begin{itemize}
\item  if $p$ divides only one of $ N^+_1$ or $N^+_2$, 
          then $\varepsilon_p(\theta(\test, \bff ^\dag) )=\ep(\pi_{1,p})\ep(\pi_{2,p})$;  
\item  if $p\mid {\rm l.c.m.}(N^+_1, N^+_2)$ and $\ep(\pi_{1,p})=\ep(\pi_{2,p})$, 
          then $\varepsilon_p(\theta(\test, \bff ^\dag) )=\ep(\pi_{1,p})$;
\item  if $p\mid N^-$ and $\ep(\pi_{1,p})=\ep(\pi_{2,p})$, 
           then $\varepsilon_p(\theta(\test, \bff ^\dag) )=-\ep(\pi_{1,p})$.
\end{itemize}  
\end{prop}
\begin{proof}
Assume that $p\mid N_1$ and $p\nmid N_2$. 
In this case, we have $\ep(\pi_{2,p}) = 1$.      
Put $h_0 = \varrho( \pMX{0}{-1}{p}{0} ,1) \in H^0(\Q_p)$. 
Then, by the definition of $W_p$, we have 
\begin{align*}
     W_p \theta(g; \test, \bff ^\dag) 
 = \int_{[H^0_1]} \sum_{x\in \bfX}  
    \langle  \omega(hh^\prime h_0, g \pMX{}{-\bfone_2}{p\bfone_2}{} )\test(x),  
    \bff (hh^\prime h_0) 
    \rangle_\cW
     dh, 
     \quad (\nu(h^\prime) = \nu(g).)
\end{align*}
We compute 
$ \omega( h_0, \pMX{}{-\bfone_2}{p\bfone_2}{} )\test(x)  
  = p^2 \widehat{\test}(h^{-1}_0 x)$,    
where the Fourier transform $\widehat{\test}$ at $p$ of $\test$ 
with respect to the self-dual Haar measure on $V^{\oplus 2}_p$,
which is explicitly given in \cite[Section 3.4]{hn15}. 
It is easy to see that  
\begin{align*}
\widehat{\test}(x) 
   = p^{-2} {\mathbb I}_{(R^\ast_p)^{\oplus 2}}(x), \quad 
  (R^\ast_p := \begin{pmatrix} \Z_p & p^{-1} \Z_p \\ \Z_p & \Z_p \end{pmatrix}). 
\end{align*}
Hence, we find that 
\begin{align*}
\omega( h_0, \pMX{}{-\bfone_2}{p\bfone_2}{} )\test(x)
  = {\mathbb I}_{(R^\ast_p)^{\oplus 2}}(h^{-1}_1x)
  = \test(x).
\end{align*}
By \cite[3.2.2 Theorem]{sc02}, we have 
$\bff ^\dag (hh^\prime h_0) = \ep(\pi_{1,p})\bff ^\dag (hh^\prime)$. 
This proves the statement. 

Both cases that  $p\nmid N_1, p \mid N_2$ and that $p$ divides ${\rm l. c. m.} (N^+_1, N^+_2)$   
   are proved in the same way with the above argument. 

Assume that $p$ divides $N^-$.
Since $N^-$ is square-free, 
there exist an unramified quadratic character $\mu_i : {\Q}^\times_p \to \C^\times$ 
such that $\pi_{i,p} \cong \mu_i \circ {\rm n}$. 
Let $h_1$ (resp. $h_2$) be an element of $D^\times_p$ 
such that ${\rm n}(h_1) = p$ (resp. ${\rm n}(h_2) =1$). 
Put $h_0=\varrho( (h_1,h_2) ,1)$. 
In the same way as above, we compute 
$ \omega( h_0, \pMX{}{-\bfone_2}{p\bfone_2}{} )\test(x)  
  = p^2 \widehat{\test}(h^{-1}_0 x)$, 
where $\widehat{\test}$ is the Fourier transform at $p$ with respect to 
the self-dual Haar measure on $V^{\oplus 2}_p$ of $\test$. 
Put $R^\ast_{0,p} = \{ y \in D_0 : (x, y) \in \Z_p, \text{ for } x \in R_{0,p}  \}$. 
Then,  it is known that $R^\ast_{0,p} = R_{0,p} h_1$
(see \cite[(25.7) Theorem]{re75}). 
Hence, we find that 
\begin{align*}
    \widehat{\test}(x) 
    = {\rm vol}(d\mu,  R_{0,p} h_1 )^2  {\mathbb I}_{(R_{0,p} h_1)^{\oplus 2}}(x)  
    = p^{-2}\test(h_0 x). 
\end{align*}
This proves 
$ \omega( h_0, \pMX{}{-\bfone_2}{p\bfone_2}{} )\test(x)  
   = \test(x)$.
Since $\pi_{i,p} \cong \mu_i \circ {\rm n}$, we see that 
$\bff ^\dag(hh_0) = \mu_1(p) \bff ^\dag(h)$. 
Since the local root number $\ep(\pi_{i,p})$ is given by $-\mu_i(p)$, 
we obtain the identity in the statement. 
\end{proof}

\begin{rem}
\begin{enumerate}
\item 
Suppose that $p\mid N$ is split. 
As already seen in Remark \ref{U(p)evrem}, 
if $\Pi^{\Gamma_0(p)}_p\neq 0$, 
then $\Pi_p$ is either type (IIa), (IVc), (VIa) or (VIb) 
     and $\dim_\C \Pi^{\Gamma_0(p)}_p =1$. 
In these cases, the eigen values of $W_p$ are also given in \cite[Table A.15]{rs07}. 
\item If $\ep(\pi_{1,p}) \neq \ep(\pi_{2,p})$ for $p\mid{\rm l.c.m.}(N_1, N_2)$ which is split, 
          then $\Pi^{\Gamma_0(p)}_p=0$ by \cite[Table 1]{jlr12} and \cite[Table A.15]{rs07}. 
          Hence, it is not necessary to consider this case in Proposition \ref{ALTheta}.
\item Suppose that $p\mid N^+$ is inert. 
         In this case, if $\Pi_p\neq 0$, 
         then $\dim_{\C} \Pi^{\Gamma_0(p)}_p=2$. 
         By \cite[Table A.15]{rs07}, we find that 
         there exists $v_\varepsilon \in \Pi_p$ such that $W_pv_\varepsilon = \varepsilon v_\varepsilon$
         for each $\varepsilon = \pm 1$. 
         This vector $v_\varepsilon$ is explicitly given by 
         $\theta(\test, \bff ^\dag) + \varepsilon W_p\theta(\test, \bff ^\dag)$. 
         We also note that, by Proposition \ref{thetaeigen} (\ref{thetaeigen(3)}), 
         \begin{align*}
            U_1(p) ( \theta(\test, \bff ^\dag) + \varepsilon W_p\theta(\test, \bff ^\dag) ) 
          = \varepsilon p ( \theta(\test, \bff ^\dag) + \varepsilon W_p\theta(\test, \bff ^\dag) ).  
         \end{align*}   
\end{enumerate}
\end{rem}




For reader's convenience, we summarize  admissible representations $\Pi_p$ 
of ${\rm GSp}_4(\Q_p)$ attached to Yoshida lifts which are discussed in this paper, as follows:

\begin{prop}\label{ThetaRepProp}
For the case that $F$ is a real quadratic field, we put $N^+_1=N^+_2=N^+$. 
We assume that 
Then, $\Pi_v$ is described as follows: 
\begin{enumerate}
\item Assume that $v=w_1w_2$ is split in $F/\Q$.
\begin{enumerate}
\item\label{Theta1a} If $v\nmid N$, write $\pi_i=\pi(\mu_i,\nu_i)$ for $i=1,2$. 
         \begin{enumerate}     
           \item\label{Theta1ai} If $\mu_2\nu^{-1}_1\neq |\cdot |^\pm$ and $\nu_2\mu^{-1}_1\neq |\cdot |^\pm$, $\Pi_v$ is type (I);
           \item\label{Theta1aii} If either $\mu_2\nu^{-1}_1= |\cdot |^\pm$ or $\nu_2\mu^{-1}_1= |\cdot |^\pm$,  $\Pi_v$ is type (IIIb).
         \end{enumerate} 
\item\label{Theta1b} If $v\mid N^-$, write $\pi_i=\sigma(\mu_i|\cdot|^{\frac{1}{2}}, \mu_i|\cdot|^{-\frac{1}{2}})$ for $i=1,2$. 
         \begin{enumerate}     
           \item\label{Theta1bi} If $\mu_1=\mu_2$, $\Pi_v$ is type (VIb);
           \item\label{Theta1bii} If $\mu_1\neq\mu_2$, $\Pi_v$ is type (Vb$^\ast$).
         \end{enumerate} 
\item\label{Theta1c} If either $v\mid N^+_1, v\nmid N^+_2$ or $v\nmid N^+_1, v\mid N^+_2$, 
         we may assume that $\pi_1=\pi(\mu_1,\nu_1)$ and $\pi_2=\sigma(\mu_2|\cdot|^{\frac{1}{2}}, \mu_2|\cdot|^{-\frac{1}{2}})$. 
         \begin{enumerate}     
           \item\label{Theta1ci} If $\mu_2\nu^{-1}_1\neq|\cdot|^{\pm\frac{3}{2}}$, $\Pi_v$ is type (IIa);
           \item\label{Theta1cii} If $\mu_2\nu^{-1}_1=|\cdot|^{\pm\frac{3}{2}}$, $\Pi_v$ is type (IVc).
         \end{enumerate} 
\item\label{Theta1d} If  $v\mid N^+_i$ for $i=1,2$, write $\pi_i=\sigma(\mu_i|\cdot|^{\frac{1}{2}},\mu_i|\cdot|^{-\frac{1}{2}})$.
         \begin{enumerate}
           \item\label{Theta1di} If $\mu_1=\mu_2$, $\Pi_v$ is type (VIa);
           \item\label{Theta1dii} If $\mu_1\neq \mu_2$, $\Pi_v$ is type (Va).  
         \end{enumerate}
\end{enumerate}
\item Assume that $v$ is non-split in $F/\Q$.
         If $\mu$ is a Galois invariant character, then $\widehat{\mu}$ denotes a character of $\Q^\times_v$ such that $\mu = \widehat{\mu}\circ{\rm N}_{F/\Q}$.
\begin{enumerate}
\item\label{Theta2a} If $v\nmid N$,  $\Pi_v$ is type (I).
\item\label{Theta2b} If  $v\mid N^+$, write $\pi=\sigma(\mu|\cdot|^{\frac{1}{2}},\mu|\cdot|^{-\frac{1}{2}})$ with $\mu=\mu^\sigma$.
         \begin{enumerate}
           \item\label{Theta2bi} If $\widehat{\mu}^2$ is trivial, $\Pi_v$ is type (Va);
           \item\label{Theta2bii} If $\widehat{\mu}^2=\eta_{F/\Q}$, $\Pi_v$ is type (IIIa).
         \end{enumerate}
\end{enumerate}
\end{enumerate}
In particular, type (I), (IIa), (IIIa), (Va), (VIa), (IXa) are generic. 
Type (IIIb), (IVc), (Vb$^\ast$), (VIb) are non-generic.
Only type (Vb$^\ast$) is supercuspidal.
\end{prop}
\begin{proof}
 We note that characters appearing here are all unramified, since our initial automorphic representations have square-free level with the trivial central character. 
In particular, if $F/\Q$ is non-split, these characters are Galois invariant. 
We also note that, by \cite[Theorem A.9, Theorem A.10, Theorem A.11]{gi11},
 $\Pi_v$ is supercuspidal if and only if $v\mid N^-$ is split 
      and the local root numbers $\ep(\pi_{1, v})$ and $\ep(\pi_{2,v})$ 
      of $\pi_{1,v}$ and $\pi_{2,v}$ respectively does not coincide. 
Then, the statement follows from \cite[Table 1]{jlr12}.
\end{proof}
